ILDAE: Instance-Level Difficulty Analysis of Evaluation Data

Knowledge of questions' difficulty level helps a teacher in several ways, such as estimating students' potential quickly by asking carefully selected questions and improving quality of examination by modifying trivial and hard questions. Can we extract such benefits of instance difficulty in NLP? To this end, we conduct Instance-Level Difficulty Analysis of Evaluation data (ILDAE) in a large-scale setup of 23 datasets and demonstrate its five novel applications: 1) conducting efficient-yet-accurate evaluations with fewer instances saving computational cost and time, 2) improving quality of existing evaluation datasets by repairing erroneous and trivial instances, 3) selecting the best model based on application requirements, 4) analyzing dataset characteristics for guiding future data creation, 5) estimating Out-of-Domain performance reliably. Comprehensive experiments for these applications result in several interesting findings, such as evaluation using just 5% instances (selected via ILDAE) achieves as high as 0.93 Kendall correlation with evaluation using complete dataset and computing weighted accuracy using difficulty scores leads to 5.2% higher correlation with Out-of-Domain performance. We release the difficulty scores and hope our analyses and findings will bring more attention to this important yet understudied field of leveraging instance difficulty in evaluations.

==> tables/efficient_eval.tex <==
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|lll|lll|lll|lll}
\toprule
\multicolumn{1}{c}{\textbf{Dataset}} &
\multicolumn{3}{c}{\textbf{0.5\%}} &
\multicolumn{3}{c}{\textbf{1\%}} &
\multicolumn{3}{c}{\textbf{2\%}} &
\multicolumn{3}{c}{\textbf{5\%}} \\
% \multicolumn{3}{c}{\textbf{$10\%$}} &
% \multicolumn{3}{c}{\textbf{$20\%$}} \\
  
%   \multicolumn{8}{c}{\textbf{Instance-Level}} &
%   \multicolumn{4}{c}{\textbf{Dataset-Level}} \\
% \multicolumn{1}{c}{} &
%   \multicolumn{2}{l}{} &
%   \multicolumn{2}{l}{\underline{Heterogeneous(B)}} &
%   \multicolumn{2}{l}{\underline{Uniform}} &
%   \multicolumn{2}{l}{\underline{Distribution (D)}} &
%   \multicolumn{2}{l}{\underline{D with $frac$=0.4}} &
%   \multicolumn{2}{l}{\underline{Random Order(B)}} &
%   \multicolumn{2}{l}{\underline{Proposed Order}} \\
  
\multicolumn{1}{c}{} & R & L & P & R & L & P & R & L & P & R & L & P  \\


\midrule
% order - paws qqp, qqp, dnli, paws wiki cola, swag, snli, mnli, adv nli, qnli, sst2, rte, arpc, agnews, emotions, arc, abductive, winogrande, csqa, quarel, quartz, socialiqa 

PAWS QQP & $-$ & $-$ & $-$ & $0.13 \pm 0.24$ & $0.36 \pm 0.05$ & $0.34 \pm 0.13$ & $0.38 \pm 0.11$ & $0.47 \pm 0.06$ & $0.55 \pm 0.19$ & $0.63 \pm 0.1$ & $0.66 \pm 0.04$ & $0.8 \pm 0.05$ \\ 

QQP & $0.63 \pm 0.06$ & $0.64 \pm 0.05$ & $0.65 \pm 0.05$ & $0.74 \pm 0.03$ & $0.74 \pm 0.01$ & $0.77 \pm 0.06$ & $0.76 \pm 0.03$ & $0.8 \pm 0.01$ & $0.84 \pm 0.04$ & $0.84 \pm 0.01$ & $0.84 \pm 0.01$ & $0.9 \pm 0.04$ \\ 

DNLI & $0.58 \pm 0.05$ & $0.59 \pm 0.1$ & $0.58 \pm 0.11$ & $0.68 \pm 0.1$ & $0.71 \pm 0.04$ & $0.76 \pm 0.07$ & $0.78 \pm 0.04$ & $0.79 \pm 0.03$ & $0.84 \pm 0.04$ & $0.88 \pm 0.01$ & $0.85 \pm 0.03$ & $0.92 \pm 0.05$ \\ 

PAWS Wiki & $0.67 \pm 0.07$ & $0.68 \pm 0.04$ & $0.78 \pm 0.06$ & $0.73 \pm 0.05$ & $0.78 \pm 0.02$ & $0.86 \pm 0.05$ & $0.84 \pm 0.0$ & $0.84 \pm 0.02$ & $0.89 \pm 0.02$ & $0.88 \pm 0.02$ & $0.91 \pm 0.02$ & $0.91 \pm 0.03$ \\ 

COLA & $-$ & $-$ & $-$ & $-0.01 \pm 0.18$ & $0.25 \pm 0.26$ & $0.24 \pm 0.45$ & $0.19 \pm 0.17$ & $0.3 \pm 0.16$ & $0.41 \pm 0.41$ & $0.53 \pm 0.09$ & $0.53 \pm 0.02$ & $0.63 \pm 0.23$ \\ 

SWAG & $0.72 \pm 0.04$ & $0.66 \pm 0.02$ & $0.75 \pm 0.06$ & $0.79 \pm 0.03$ & $0.77 \pm 0.03$ & $0.78 \pm 0.05$ & $0.86 \pm 0.02$ & $0.83 \pm 0.04$ & $0.86 \pm 0.03$ & $0.92 \pm 0.01$ & $0.91 \pm 0.02$ & $0.89 \pm 0.02$ \\ 


SNLI & $0.55 \pm 0.09$ & $0.38 \pm 0.17$ & $0.68 \pm 0.13$ & $0.68 \pm 0.05$ & $0.58 \pm 0.08$ & $0.78 \pm 0.08$ & $0.77 \pm 0.04$ & $0.78 \pm 0.02$ & $0.83 \pm 0.04$ & $0.83 \pm 0.02$ & $0.85 \pm 0.02$ & $0.88 \pm 0.04$ \\ 

MNLI & $0.7 \pm 0.04$ & $0.71 \pm 0.03$ & $0.73 \pm 0.07$ & $0.8 \pm 0.02$ & $0.8 \pm 0.04$ & $0.82 \pm 0.08$ & $0.87 \pm 0.01$ & $0.86 \pm 0.02$ & $0.89 \pm 0.03$ & $0.9 \pm 0.01$ & $0.91 \pm 0.02$ & $0.93 \pm 0.02$ \\ 



Adv. NLI R1 & $0.0 \pm 0.08$ & $-0.07 \pm 0.06$ & $0.17 \pm 0.27$ & $0.02 \pm 0.13$ & $0.09 \pm 0.11$ & $0.08 \pm 0.2$ & $-0.1 \pm 0.22$ & $0.14 \pm 0.14$ & $0.13 \pm 0.18$ & $0.1 \pm 0.12$ & $0.19 \pm 0.2$ & $0.3 \pm 0.18$ \\ 

Adv. NLI R2 & $-0.08 \pm 0.04$ & $-0.01 \pm 0.06$ & $-0.08 \pm 0.16$ & $-0.08 \pm 0.07$ & $0.02 \pm 0.03$ & $-0.03 \pm 0.21$ & $0.01 \pm 0.04$ & $0.06 \pm 0.14$ & $0.0 \pm 0.12$ & $0.1 \pm 0.13$ & $0.17 \pm 0.03$ & $0.17 \pm 0.03$ \\ 

Adv. NLI R3 & $-0.15 \pm 0.12$ & $0.15 \pm 0.1$ & $0.1 \pm 0.21$ & $-0.03 \pm 0.06$ & $0.07 \pm 0.1$ & $0.1 \pm 0.11$ & $-0.08 \pm 0.11$ & $0.13 \pm 0.08$ & $0.18 \pm 0.16$ & $0.06 \pm 0.1$ & $0.07 \pm 0.1$ & $0.12 \pm 0.17$ \\ 

QNLI & $0.41 \pm 0.1$ & $0.44 \pm 0.04$ & $0.48 \pm 0.13$ & $0.57 \pm 0.04$ & $0.55 \pm 0.1$ & $0.57 \pm 0.07$ & $0.67 \pm 0.03$ & $0.64 \pm 0.06$ & $0.7 \pm 0.06$ & $0.76 \pm 0.01$ & $0.79 \pm 0.01$ & $0.78 \pm 0.06$ \\ 





SST-2 & $-$ & $-$ & $-$ & $0.08 \pm 0.15$ & $0.16 \pm 0.35$ & $0.29 \pm 0.25$ & $0.25 \pm 0.21$ & $0.18 \pm 0.14$ & $0.4 \pm 0.2$ & $0.56 \pm 0.05$ & $0.47 \pm 0.07$ & $0.52 \pm 0.16$ \\ 

RTE & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $0.17 \pm 0.14$ & $0.13 \pm 0.12$ & $-0.05 \pm 0.38$ & $0.31 \pm 0.16$ & $0.28 \pm 0.08$ & $0.26 \pm 0.32$ \\ 


MRPC & $0.04 \pm 0.09$ & $-0.03 \pm 0.18$ & $0.21 \pm 0.16$ & $-0.02 \pm 0.09$ & $0.05 \pm 0.2$ & $0.29 \pm 0.21$ & $0.24 \pm 0.15$ & $0.1 \pm 0.08$ & $0.36 \pm 0.15$ & $0.38 \pm 0.09$ & $0.26 \pm 0.18$ & $0.45 \pm 0.08$ \\ 

AgNews & $0.12 \pm 0.26$ & $0.14 \pm 0.27$ & $0.47 \pm 0.05$ & $0.25 \pm 0.34$ & $0.41 \pm 0.14$ & $0.52 \pm 0.1$ & $0.54 \pm 0.2$ & $0.49 \pm 0.07$ & $0.65 \pm 0.07$ & $0.71 \pm 0.02$ & $0.62 \pm 0.03$ & $0.75 \pm 0.06$ \\ 

Emotions & $0.25 \pm 0.11$ & $0.18 \pm 0.19$ & $0.29 \pm 0.27$ & $0.34 \pm 0.1$ & $0.24 \pm 0.19$ & $0.22 \pm 0.2$ & $0.41 \pm 0.13$ & $0.3 \pm 0.17$ & $0.29 \pm 0.22$ & $0.51 \pm 0.15$ & $0.42 \pm 0.14$ & $0.55 \pm 0.11$ \\ 

ARC Easy & $-$ & $-$ & $-$ & $0.0 \pm 0.2$ & $-0.03 \pm 0.12$ & $0.42 \pm 0.19$ & $0.22 \pm 0.08$ & $0.2 \pm 0.13$ & $0.47 \pm 0.19$ & $0.34 \pm 0.13$ & $0.43 \pm 0.05$ & $0.59 \pm 0.13$ \\ 

ARC Diff & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-0.12 \pm 0.16$ & $-0.15 \pm 0.1$ & $0.15 \pm 0.29$ & $-0.09 \pm 0.2$ & $-0.1 \pm 0.15$ & $0.28 \pm 0.13$ \\ 



Abductive NLI & $0.08 \pm 0.26$ & $0.17 \pm 0.05$ & $0.16 \pm 0.09$ & $0.19 \pm 0.19$ & $0.26 \pm 0.08$ & $0.3 \pm 0.07$ & $0.37 \pm 0.08$ & $0.31 \pm 0.1$ & $0.42 \pm 0.13$ & $0.49 \pm 0.06$ & $0.33 \pm 0.1$ & $0.57 \pm 0.08$ \\ 

Winogrande & $-0.19 \pm 0.11$ & $-0.03 \pm 0.06$ & $0.0 \pm 0.17$ & $-0.11 \pm 0.09$ & $-0.05 \pm 0.12$ & $0.11 \pm 0.15$ & $-0.08 \pm 0.07$ & $-0.01 \pm 0.09$ & $0.09 \pm 0.14$ & $0.02 \pm 0.06$ & $0.03 \pm 0.07$ & $0.03 \pm 0.1$ \\ 

CSQA & $0.29 \pm 0.11$ & $0.28 \pm 0.1$ & $0.31 \pm 0.07$ & $0.36 \pm 0.14$ & $0.37 \pm 0.08$ & $0.39 \pm 0.09$ & $0.48 \pm 0.07$ & $0.44 \pm 0.04$ & $0.49 \pm 0.09$ & $0.63 \pm 0.07$ & $0.6 \pm 0.12$ & $0.69 \pm 0.08$ \\ 

QuaRel & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $0.03 \pm 0.29$ & $-0.08 \pm 0.14$ & $0.32 \pm 0.26$ & $0.24 \pm 0.12$ & $0.25 \pm 0.15$ & $0.33 \pm 0.25$ \\ 

QuaRTz & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $0.14 \pm 0.12$ & $0.13 \pm 0.07$ & $0.34 \pm 0.19$ & $0.16 \pm 0.14$ & $0.13 \pm 0.05$ & $0.36 \pm 0.04$ \\ 

SocialIQA & $0.19 \pm 0.09$ & $0.15 \pm 0.29$ & $0.37 \pm 0.17$ & $0.34 \pm 0.07$ & $0.28 \pm 0.21$ & $0.4 \pm 0.09$ & $0.49 \pm 0.06$ & $0.46 \pm 0.11$ & $0.58 \pm 0.1$ & $0.57 \pm 0.09$ & $0.63 \pm 0.04$ & $0.67 \pm 0.04$ \\ 

\bottomrule
\end{tabular}}
\caption{\Neeraj{Needs to be presented better} Kendall correlation with the full evaluation dataset evaluation achieved by various approaches with different percentage of instances selected for evaluation. R, L, and P correspond to results of Random, Length, and Proposed approach. $-$ indicate that not even a single instance could be selected. Each cell shows the mean and standard deviation obtained obtained from 5 different runs.}
\Swaroop{Suggestion: Divide into multiple tables or make a full page table}
\label{tab:efficiency}
\end{table*}

==> tables/instance_selection_techniques.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{p{2.3cm}p{2cm}p{1.9cm}}
    \toprule
        \textbf{Technique} & \textbf{\#Evaluations}  & \textbf{Parameters} \\
        \midrule
        % \midrule
        \textbf{Standard} & $N$ & -\\
        \midrule
        \textbf{by 2} & $N/2$ & -\\
        \textbf{by 2} & $N/2$ & -\\
        \textbf{by 2} & $N/2$ & -\\
        \textbf{by 2} & $N/2$ & -\\
        
        
        
    \bottomrule
    \end{tabular}
    \caption{Comparison of various instance selection techniques based on the number of evaluations required for $N$ test instances.}
    \label{tab:instace_selection}
\end{table}

